Analyzing and Improving Fault Tolerance of Learning-Based Navigation Systems

Learning-based navigation systems are widely used in autonomous applications, such as robotics, unmanned vehicles and drones. Specialized hardware accelerators have been proposed for high-performance and energy-efficiency for such navigational tasks. However, transient and permanent faults are increasing in hardware systems and can catastrophically violate tasks safety. Meanwhile, traditional redundancy-based protection methods are challenging to deploy on resource-constrained edge applications. In this paper, we experimentally evaluate the resilience of navigation systems with respect to algorithms, fault models and data types from both RL training and inference. We further propose two efficient fault mitigation techniques that achieve 2x success rate and 39% quality-of-flight improvement in learning-based navigation systems.

==> extension.tex <==
\section*{Extension}


% Extension:
% 1. From inference to training:

% (1) characterize fault tolerance of RL training process 

% (2) robust training: add some resilient features during RL training (eg. loss function), applied FI in trained models (compare w/ and w/o resilient features)

% 2. From single drone to multi-drone system:

% (1) compute: hardware faults 

% (2) communication

% 3. Error protection mechanism (regularizer, anomaly detection, autoencoder, checksum, etc.)
